PointRWKV: Efficient RWKV-Like Model for Hierarchical Point Cloud Learning

Transformers have revolutionized the point cloud learning task, but the quadratic complexity hinders its extension to long sequence and makes a burden on limited computational resources. The recent advent of RWKV, a fresh breed of deep sequence models, has shown immense potential for sequence modeling in NLP tasks. In this paper, we present PointRWKV, a model of linear complexity derived from the RWKV model in the NLP field with necessary modifications for point cloud learning tasks. Specifically, taking the embedded point patches as input, we first propose to explore the global processing capabilities within PointRWKV blocks using modified multi-headed matrix-valued states and a dynamic attention recurrence mechanism. To extract local geometric features simultaneously, we design a parallel branch to encode the point cloud efficiently in a fixed radius near-neighbors graph with a graph stabilizer. Furthermore, we design PointRWKV as a multi-scale framework for hierarchical feature learning of 3D point clouds, facilitating various downstream tasks. Extensive experiments on different point cloud learning tasks show our proposed PointRWKV outperforms the transformer- and mamba-based counterparts, while significantly saving about 42\% FLOPs, demonstrating the potential option for constructing foundational 3D models.

==> Makefile <==
main:
	pdflatex main

full:
	pdflatex main && \
	bibtex main && \
	pdflatex main && \
	pdflatex main

camready: full
	gs -dNOPAUSE -dBATCH -dNOPLATFONTS -sDEVICE=pdfwrite -dEmbedAllFonts=true -sOutputFile=main-gs.pdf -f main.pdf

cut: full
	pdftk main.pdf cat 1-11 output main_submit.pdf
	pdftk main.pdf cat 12-end 9-11 output suppl_submit.pdf

clean:
	rm *.aux *.bbl *.blg *.log *.pdf *.dep *.brf *.fls *.out

run:
	evince main.pdf

compress:
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/default -dNOPAUSE -dQUIET -dBATCH -dDetectDuplicateImages -dCompressFonts=true -r150 -sOutputFile=suppl.pdf suppl_highRes.pdf

arxiv: full
	rm -rf ../arxiv.tar.gz ../paper_arXiv
	cd ../arxiv-latex-cleaner && python3.9 -m arxiv_latex_cleaner ../paper/
	# Unfortunately it still doesn't remove unused PDF etc files... need to use the arxiv-collector
	rm -f /tmp/latexmk
	cd .. && python3.9 arxiv-collector/arxiv_collector.py --get-latexmk /tmp/latexmk
	cd ../paper_arXiv && python3.9 ../arxiv-collector/arxiv_collector.py --latexmk /tmp/latexmk main.tex
	mv ../paper_arXiv/arxiv.tar.gz ../
	rm -rf ../paper_arXiv


